Neural heuristics for SAT solving

We use neural graph networks with a message-passing architecture and an attention mechanism to enhance the branching heuristic in two SAT-solving algorithms. We report improvements of learned neural heuristics compared with two standard human-designed heuristics.

==> algorithm.tex <==
\section{Main algorithm}

% from https://tex.stackexchange.com/questions/163768/write-pseudo-code-in-latex
\begin{algorithm}[H]
\caption{Simplified propositional SAT algorithm}\label{dpll}
\begin{algorithmic}[1]
\Function{DPLL}{$\Phi$}
\If {$\Phi \text{ is empty}$} \Return True
\EndIf
\If {$\Phi \text{ contains an empty clause}$} \Return False
\EndIf
\State $l \gets \text{choose-literal}(\Phi)$
\State\Return {DPLL($\Phi \wedge l$) or DPLL($\Phi \wedge \text{not }l$)}
\EndFunction
\end{algorithmic}
\label{backtracking}
\label{alg:backtracking}
\end{algorithm}

Pseudocode + precise information where the non-deterministic choice happens

\begin{itemize}
    \item  DPLL description
\item main loop slide?
\item simplified SAT algorithm (aka simplified DPLL),
\item input:  CNF formula
\item pseudocode with choose-literals left ambiguous
\item note: reduces the problem by one variable at each level (but returns to the higher level if fails to find a solution)
\item goal: Learned policy which outdoes basic heuristics and generalises to larger instances than these in training
\item SAT algorithm with heuristic/oracle/policy (in slides: embedding - probably not relevant without EqNet)

\end{itemize}



Handbook of Satisfiability???
Other sources about heuristics for DPLL (maybe from papers
accompanying \url{http://fmv.jku.at/picosat/} \url{minisat.se/Papers.html}

==> attention_table.tex <==

\begin{tabular}{|l|rrr|rrr|}
\hline
\multirow{2}{*}{Problem} &
\multicolumn{3}{c|}{Attention disabled} &
\multicolumn{3}{c|}{Attention enabled} \\
% \hline  % doesn't work easily with multirow
&
loss &
{\it sat} error &
{\it policy} error &
loss &
{\it sat} error &
{\it policy} error \\
\hline
SR(30), level 20 &
\bf{21.370±0.295} &
\bf{0.178±0.017} &
\bf{0.091±0.006} &
22.260±0.550 &
0.210±0.017 &
0.093±0.005 \\
SR(30), level 30 &
28.795±0.539 &
0.101±0.008 &
0.059±0.003 &
\bf{28.178±0.672} &
\bf{0.084±0.004} &
\bf{0.050±0.002} \\
SR(50), level 20 &
23.040±0.044 &
0.297±0.005 &
0.125±0.001 &
\bf{22.512±0.138} &
\bf{0.259±0.016} &
\bf{0.112±0.004} \\
SR(50), level 30 &
32.186±0.132 &
0.281±0.003 &
0.118±0.001 &
\bf{32.024±0.555} &
\bf{0.233±0.017} &
\bf{0.105±0.006} \\
SR(50), level 40 &
41.457±0.401 &
\bf{0.183±0.015} &
0.092±0.007 &
\bf{39.397±0.166} &
0.187±0.004 & 
\bf{0.090±0.002} \\
SR(70), level 20 &
23.794±0.062 &
0.350±0.005 &
0.135±0.000 &
\bf{23.574±0.177} &
\bf{0.333±0.016} &
\bf{0.127±0.002} \\
SR(70), level 30 &
34.088±0.070 &
0.304±0.003 &
0.125±0.002 &
\bf{33.010±0.482} & 
\bf{0.266±0.033} & 
\bf{0.110±0.007} \\
\hline
\end{tabular}

==> table_1000_steps.tex <==
\begin{table}
\resizebox{\textwidth}{!}{%
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} \hline
    guidance &	SR(16)	& SR(18) & SR(20) & SR(25) & SR(30) & SR(40) & SR(50) & SR(70) & SR(90)\\ \hline
hybrid SR(8) &	{\bf 99} & 83 & {\bf 76} & 57 & 49 & 22 & 23 & 11 & 2\\
hybrid SR(30) &	93	& 89 & 71 & 58 & 42 & 25 & 12 & 6 & 0 \\
hybrid SR(50) & 93	& {\bf 90} & 65 & {\bf 61} & {\bf 53} & {\bf 46} & {\bf 30} & {\bf 19} & {\bf 16}\\
hybrid SR(100) & 94	& 85 & 68 & 58 & 31	& 25 & 6 & 4 & 2\\
mostcommon  & {\bf 99} & {\bf 90} & 60	& 26 & 10 & 5 & 3 & 0 & 0\\ \hline
    \end{tabular}}
    \caption{Problems solved in 1000 steps using various DPLL heuristics. In the first row we consider guidance trained on the SR(8) dataset and test it against SR(n) up to $n=90$. In subsequent row we test other instances of guidance. Compare with Table \ref{tab:1e6steps} in the Appendix.}
    \label{tab:1e3steps}
\end{table}

==> table_architecture.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c c c}\hline \\
size & 	number & parameters \\ \hline
1	& 2	& 2 \\
128	& 10 & 	1280 \\
32768	& 1	& 32768 \\
16384 &	4 &	65536 \\
49152 & 1 & 49152 \\ \hline
    \end{tabular}
    \caption{The table lists all layers present in our implementation of the message passing architecture. The left column lists  sizes of layers and the center column lists corresponding numbers of layers. In total the network has $148738$ parameters.}
    \label{tab:mp_architectures}
\end{table}



==> table_cdcl_steps.tex <==
\begin{tabular}{lrrrrr}
Guidance & SR(40) & SR (50) & SR(60) & SR(70) & SR(90) \\
\hline
JW-OS & 34.17±18.73 & 75.53±67.41 & \textbf{144.67±113.02} & \textbf{215.00±217.21} & 851.00±806.57 \\
Humble (ours) & \textbf{32.80±42.92} & \textbf{49.60±60.84} & 162.13±215.26 & 309.17±406.07 & \textbf{523.77±651.80} \\
$SR(50)$ (ours) & 49.37±85.94 & 86.53±142.90 & 493.50±725.35 & 1061.13±1575.44 & -
\end{tabular}

==> table_dpll_steps.tex <==
\begin{tabular}{lrrrrrrr}
Guidance & SR(10) & SR(20) & SR (30) & SR(40) & SR(50) & SR(70) & SR(90) \\
\hline
DLIS & 8.14±3.90 & 23.56±17.36 & 53.31±48.86 & 190.63±167.22 & 514.93±439.86 & 3431.60±3416.16 & 24625.23±17007.14 \\
JW-OS & 7.33±3.55 & 18.65±11.41 & 32.82±26.21 & 84.10±73.23 & 152.00±146.38 & \textbf{614.37±708.74} & 3088.50±2859.22 \\
Humble & \textbf{5.56±1.86} & \textbf{15.43±15.85} & \textbf{28.40±45.56} & \textbf{71.88±132.42} & \textbf{113.67±188.37} & 1034.70±1554.57 & \textbf{3057.73±4517.29} \\
$SR(50)$ & 5.64±2.56 & 17.83±22.51 & 42.46±79.51 & - & - & - & -
\end{tabular}

==> table_loss_sr8.tex <==
%\begin{table}
%    \centering

\resizebox{\textwidth}{!}{%
    \begin{tabular}{c c c c c}\hline
iteration & policy loss & sat loss & policy error & sat error \\
\hline
1	& 0.69	& 0.69 &	0.47	& 0.45 \\
2 & 0.69 & 0.69 & 0.39 & 0.48 \\
3 & 0.67 &	0.7	& 0.36	& 0.48 \\ 
4 & 0.65 &	0.79 &	0.31 &	0.54 \\
5 & 0.63 &	0.69 &	0.3	& 0.47 \\ 
6 & 0.63 &	0.76 &	0.29 &	0.44 \\
7 & 0.58 &	0.71 &	0.26 &	0.4 \\
8 & 0.56 &	0.62 &	0.23 &	0.33 \\
9 & 0.53 &	0.56 &	0.2	& 0.29 \\
10 & 0.51 &	0.56 &	0.18 &	0.26 \\
11 & 0.48 &	0.48 &	0.14 &	0.19 \\ 
12 & 0.46 &	0.43 &	0.13 &	0.16 \\
13 & 0.45 &	0.4	& 0.12	& 0.14 \\
14 & 0.43 &	0.36 & 	0.09 &	0.14 \\
15 & 0.43 &	0.3	& 0.09	& 0.13 \\
16 & 0.41 &	0.3	& 0.07	& 0.11 \\
17 & 0.4 &	0.27 &	0.07 &	0.09 \\
18 & 0.39 &	0.23 &	0.06 &	0.08 \\
19 & 0.38 &	0.24 &	0.05 &	0.07 \\
20 & 0.38 &	0.22 &	0.05 &	0.05\\
    \end{tabular}}
% \end{table}


==> table_steps.tex <==

\begin{table}[H]
    \centering
    
\resizebox{\textwidth}{!}{%
    \begin{tabular}{c c c c c c c c c c c c c} \hline
model           &	SR(8)  & SR(10) & SR(12)	& SR(14) &   SR(15)     & SR(16)	&  SR(18)	& SR(20)	& SR(25)	& SR(30)	& SR(40)	& SR(50) \\ \hline
hybrid SR(8)    &	\textbf{9}  &	17 & 25	& 101 &  \textbf{85}     & \textbf{144}	& 326	& 633	& 2601	& 9964	& 158542 & 185995 \\ 
SR(8)           &	\textbf{9}  &	17 & 24 & 134 &  125	& 254	& 746	& 1671	& 10687 & NaN   & NaN  	 & NaN	\\
hybrid SR(30)   &	20 &    20 & \textbf{15}	& 173 &  172	& 298	& 339	& 783	& 5714	& 7774	& 169314 & 1893618 \\
hybrid SR(50)   &	15 &    \textbf{14} & 59	& \textbf{77} &   159	& 326	& \textbf{229}	& \textbf{485}	& \textbf{2325}	& 6692	& \textbf{29255}	 & \textbf{79886} \\
hybrid SR(100)  &	11 &	51 & 90	& 142 &  192	& 290	& 504	& 752	& 3397	& \textbf{6022}	& 54051	 & 2046069 \\
mostcommon      &	24 &	53 & 101 & 183 & 240	& 338	& 313	& 1185	& 4556	& 13566	& 1651067 & 2837835 \\
randomvar       &	65 &   144 & 270 & 538 & 862	& 1164	& 2436	& 5251	& 25275	& 125610 & 4358797 & NaN \\
randomclause    &   51 &   103 & 216 & 394 & 548	& 745	& 1363	& 2788	& 13385	& 57509	 & 1705605 & NaN \\
\hline
    \end{tabular}}
    \caption{Average number of steps over 100 trials for models listed in the right column. Models were tested on datasets SR(n) for various $n\leq 50$. NaN refers to a timeout. }
    \label{tab:proofsteps}
\end{table}






==> tables_to_diagrams.tex <==
\section{Data used in the diagrams}
To facilitate reading the data from diagrams, we include the tabular data in this section.
\begin{figure}[H]
    \centering
    \resizebox{\textwidth}{!}{%
    \input{table_dpll_steps.tex}}
    \caption{Raw data for diagram in Figure \ref{fig:steps}}
    \label{tab:steps}
\end{figure}

\begin{figure}[H]
    \centering
    \resizebox{\textwidth}{!}{%
    \input{table_cdcl_steps.tex}}
    \caption{Raw data for diagram in Figure \ref{fig:cdcl_steps}}
    \label{tab:cdcl_steps}
\end{figure}




